Tidally-induced nonlinear resonances in EMRIs with an analogue model

One of the important targets for the future space-based gravitational wave observatory LISA is extreme mass ratio inspirals (EMRIs), where long and accurate waveform modeling is necessary for detection and characterization. Modeling EMRI dynamics requires accounting for effects such as the ones induced by an external tidal field, which can break integrability at resonances and cause significant dephasing. In this paper, we use a Newtonian analogue of a Kerr black hole to study the effect of an external tidal field on the dynamics and the gravitational waveform. We have developed a numerical framework that takes advantage of the integrability of the background system to evolve it with a symplectic splitting integrator, and compute approximate gravitational waveforms to estimate the timescale over which the perturbation affects the dynamics. Comparing this timescale with the characteristic time under radiation reaction at resonance, we introduce a tool for quantifying the regime in which tidal effects might be included when modeling EMRI gravitational waves. As an application of this framework, we perform a detailed analysis of the dynamics at one resonance to show how different entry points into the resonance in phase-space can produce substantially different dynamics, and how one can estimate bounds for the parameter space where tidal effects may become dominant. Such bounds will scale as $\varepsilon \gtrsim C \, q$, where $\varepsilon$ measures the strength of the external tidal field, $q$ is the mass ratio, and $C$ is a number which depends on the resonance and the shape of the tide. We demonstrate how to estimate $C$ using our framework for the 2:3 radial to polar frequency resonance in our model system. This framework can serve as a proxy for proper modeling of the tidal perturbation in the fully relativistic case.

==> Makefile <==
# Use this makefile to produce the standalone figure if needed

.PHONY: all

# make is make all by default (first rule in Makefile)
all: figures/resonance-cartoon.pdf

figures/resonance-cartoon.pdf: figures/resonance-cartoon.tex Tidal.tex
	pdflatex -shell-escape -interaction=batchmode -jobname "resonance-cartoon" "\def\myext{1} \def\tikzexternalrealjob{Tidal}\input{tidal.tex}"
	mv resonance-cartoon.pdf figures

